Neat: Low-Complexity, Efficient On-Chip Cache Coherence

Cache coherence protocols such as MESI that use writer-initiated invalidation have high complexity and sometimes have poor performance and energy usage, especially under false sharing. Such protocols require numerous transient states, a shared directory, and support for core-to-core communication, while also suffering under false sharing. An alternative to MESI's writer-initiated invalidation is self-invalidation, which achieves lower complexity than MESI but adds high performance costs or relies on programmer annotations or specific data access patterns. This paper presents Neat, a low-complexity, efficient cache coherence protocol. Neat uses self-invalidation, thus avoiding MESI's transient states, directory, and core-to-core communication requirements. Neat uses novel mechanisms that effectively avoid many unnecessary self-invalidations. An evaluation shows that Neat is simple and has lower verification complexity than the MESI protocol. Neat not only outperforms state-of-the-art self-invalidation protocols, but its performance and energy consumption are comparable to MESI's, and it outperforms MESI under false sharing.

==> design-notes.tex <==
\section{Design}

\subsection{Base Design}

\mike{I like the design and optimizations; they seem correct and efficient to me.
We may need something more for avoiding self-invalidation in
general, e.g., for medium-length regions that saturate the write signature but
don't amortize self-invalidation costs, but I think it'd be good to design stuff
based on preliminary results.}

\mike{Rui, you mentioned that you think the design is looking kind of like DeNovoND's.
First, DeNovoND doesn't actually work with legacy programs; DeNovoND assumes that it knows which locks guard which variables.
Second, DeNovoND/DeNovo's ``registration'' seems related to deferred write-backs but also different; what do you think?}
\brandon{The lock association problem is a pretty high cost -- there has been lots of work on trying to infer that, some of which (Vaziri, et al) concluding that it is a tough mapping to figure out.  Registration is, indeed, how they handle deferred write-backs, instead of doing self-invalidate with aggressive writeback.  I think our bloom filter trick is like registration and a useful exercise might be understanding how/if they are duals of one another}

\paragraph*{Metadata.}
\begin{itemize}
\item Private line metadata -- One write bit per byte.
\end{itemize}

\paragraph*{Data Access.}
A core performs nothing special at each memory read. \brandon{This is a huge feature, but one that other work maybe also has?  A qualitatively reduced cost with (hopefully) a quantitatively huge benefit.}
For each memory write, if the write hits in the private cache, the core sets the write bits for those written-to bytes
of the line. Otherwise, the core fetches the line from the LLC. 
We don't need to handle WAR upgrades.

\paragraph*{Eviction of a private line.} 
When a line is evicted from the L1/L2 to LLC, its written-to bytes (but not its other bytes) need to be written back to the LLC. 
Note that a core performs \emph{silent} evictions for read-only lines without any communication with the LLC.

\paragraph*{Synchronization.}
When a core reaches a synchronization operation, \ie, a lock acquire or release, it performs the following actions.
\\
At acquire:
\begin{itemize}
\item \textbf{Self-invalidation} -- The core invalidates all of its private cache lines. 
If the line has its write bits set, the core needs to commit the line first, writing back dirty values and clearing write bits for the line.
\end{itemize}
~\\
At release:
\begin{itemize}
\item \textbf{Commit} -- For each dirty line, \ie, a line with write bits set,
the core writes back its written-to bytes to the LLC and clears its 
write bits.
\end{itemize}

\subsection{Opt: avoiding self-invalidation using write signatures}

\paragraph*{Metadata added.}

\begin{itemize}
\item Per-core metadata in the LLC -- A ???-bit bloom-filter as a write signature. (The
write signature may be fairly large (say, 10 times larger than the signature that'll fit in a flit).
If it's sparse, it can be communicated from the LLC to the core in a sparse format (\eg, run-length encoding or a list of bit positions).
\end{itemize}

\brandon{We borrow from TM and Bulk and others, using signatures.  We should look at Josep's papers carefully to be sure he's not using a similar Bulk summary trick to ensure DRF0.  He has a million Bulk/Sig papers.}
% \mike{Something else we discussed:
% It may make sense to have a fairly large signature (say, 10 times larger than the signature that'll fit in a flit).
% If it's sparse, it can be communicated from the LLC to the core in a sparse format (\eg, run-length encoding or a list of bit positions).
% \rui{Thanks Mike! I've included them in the above paragraph.}}

\paragraph*{Eviction of a private line.} 
The LLC updates other cores' write signatures with the evicted line. 

\paragraph*{Synchronization.}
The following changes are made to the actions that a core performs at each synchronization operation.
\\
At acquire:
\begin{itemize}
% It could use the optimization:
% \begin{itemize}
%   \item Defer write-backs of dirty lines (the LLC knows that the core is the owner; requires versions or write
%   signatures).
% \end{itemize}
\item \textbf{Self-invalidation} -- The core requests the LLC to send the updated write signature 
(and to clear the write signature for the core \brandon{Let's think about the atomicity of this operation and the operations of the executing region.}) 
and invalidates a private cache line only if the write signature shows that ownership of the line may have changed during the acquire-free region (AFR) that is ending.
% \brandon{Framing this with ownership-based coherene: ``If ownership may have changed during the region that is ending''} 
% If the line has its write bits set, the core needs to commits the line first, writing back dirty values and clearing write bits for the line.

% with the following optimizations:
% \begin{itemize}
%   \item Self-invalidation optimization. For each \emph{completely} touched line (i.e., lines with all write
%   bits set), the line is definitely valid since data-race-free is guaranteed, so the core avoids invalidating it.
%   For untouched lines and touched lines with untouched bytes, the core can avoid invalidating it if the
%   write signature (or the version) indicates no other core wrote to the line.
%   \item \emph{Cond-invalid} state (requires versions).
% \end{itemize}
% \item \textbf{Clear-write-signature} -- The core requests the LLC to clear its write signature.
% \brandon{Let's think about the atomicity of this operation and the operations of the executing region.}
% \mike{The write signature represents (other cores') writes \textbf{to the LLC} during the core's execution,
% so this operation on the write signature for the core is really done by the LLC controller (or LLC-side CC, if we have one), right?
% \rui{Yes.}}
\end{itemize}
~\\
At release:
\begin{itemize}
\item \textbf{Commit} -- The LLC updates other cores' write signatures with all newly committed lines.
\end{itemize}

\subsection{Opt: deferring write-backs of dirty lines}
\paragraph*{Metadata.}
We add a \emph{deferred-writeback} bit for each private line to indicate whether the line is a deferred line, \ie, a
line that has values whose write-backs to the LLC are deferred and an \emph{ownerID} for each shared line in the LLC to
register the owner core of each deferred line. Also, we use the write bits of each private line to indicate at which
bytes the line has the latest version of values, whenever they were written by the corresponding core.
% \mike{What does the last sentence mean?
% Based on reading the whole subsection, I think the deferred-writeback bit indicates that the LLC already knows it's the owner of the line.
% \rui{I was trying to say that what the write bits indicate is not only that a line is written in the current region at
% some bytes as in the base design, but also that the line has lastest values at corresponding bytes, whether they are
% written in the current region or previous regions. I modified the last sentence above. Does it make sense now?}}

\paragraph*{Synchronization.}
The following changes are made to the actions that a core performs at each synchronization operation.

\begin{itemize}
\item \textbf{self-invalidation} -- The core needs to ``undefer'' a deferred line before self-invalidating it, 
\ie, the core writes back the line's dirty values (and clears its write bits and deferred-writeback bit) and the LLC clears the ownerID for the line.
\\
Note that before the core writes back any dirty values (either of a deferred line or a normal dirty line), the LLC needs to fetch the line from its owner.

\item \textbf{commit} -- For each dirty line, 
the core defers writing back its dirty values
until they are needed by another core or another core wants to write back or defer the line.  The core keeps the write bits
for the line to indicate that the line has the latest version of values at corresponding bytes and also sets the
deferred-writeback bit of the line. The LLC registers the core as the owner core
of the line. 
\\
If the line has already been deferred in a previous region of the
\emph{same} core, the core doesn't need to communicate with the LLC to defer it
again.
If the line has been deferred by a \emph{different} core, it needs to be fetched
from its old owner by the LLC before being deferred by the current core.
\end{itemize}

\paragraph*{Fetching a deferred line from its owner core.}
A deferred line is fetched to the LLC from its owner core when another core requests it at a read/write miss or wants to update it on eviction, during commit or self-invalidation
(or if the owner core has to evict it). The LLC fetches
the dirty values of the line before fulfilling the request and the owner core clears the write bits and the deferred-writeback bit for the line.

\subsection{Opt: avoiding self-invalidation with a special line state}
The above design with the optimization of deferring write-backs can use an optimization to avoid self-invalidating a line until
the next read at the line's \emph{non-written-to} bytes. 

\paragraph*{Metadata.}
We add an additional state \code{Partial-invalid} for each private line to
indicate that the line might be invalid due to stale values at non-written-to
bytes, \ie, bytes with write bits unset.

\paragraph*{Data Access.}
If a core hits a line in \code{Partial-invalid} state and wants to \emph{read} any of its non-written-to bytes, 
the core needs to fetch the updated values for all these bytes from the LLC and change the line's state from \code{Partial-invalid} to \code{valid}.
\\
A core can write to any bytes or read \emph{written} bytes of a partially
invalid line directly.

\paragraph*{Synchronization.}

\begin{itemize}
\item \textbf{self-invalidation} -- If a line (might be a deferred line)
is contained in a core's write signature, the core changes the line's state to
\code{Partial-invalid}, rather than writing back and self-invalidating it.
\end{itemize}

~\\
Note that a deferred line can be in the \code{Partial-invalid} state in a core even if the core is the owner,
since ownership only ensures that a core has updated values at \emph{written} bytes.

==> figure-false-sharing.tex <==
\begin{figure*}[t!]
  \centering
  \vspace*{-2.5em}
  \hspace*{-1em}
  \subfloat[Execution time]
  {\includegraphics[width=0.3\linewidth]{figs/isca20/false_sharing/max_BandwidthDrivenCycleCountMax}\label{fig:perf-fs}}

  % \vspace*{-1.0em}
  % \hspace*{6em}\includegraphics[width=1.13\linewidth]{figs/legend_perf}
  % \vspace*{-3.0em}\\
  % \hspace*{-1em}
  % \subfloat[Execution time breakdown across all cores]
  % {\includegraphics[width=0.62\linewidth]{figs/isca20/servers/g_BandwidthDrivenCycleCount}\label{fig:perf-breakdown-servers}}

  \vspace*{-1.0em}
  \hspace*{-0.4em}
  \hspace*{7em}\includegraphics[width=0.8\linewidth]{figs/legend_energy}
  \vspace*{-1.5em}\\
  \hspace*{-1em}
  \subfloat[Energy usage of the cache and memory subsystem]
  {\includegraphics[width=0.3\linewidth]{figs/isca20/false_sharing/TotalEnergy} \label{fig:energy-fs}}

  \vspace*{-1.0em}
  \hspace*{-1em}
  \subfloat[Energy--delay product (EDP)]
  {\includegraphics[width=0.3\linewidth]{figs/isca20/false_sharing/EDP} \label{fig:edsp-fs}}

  % \mike{Fonts in graph are too small. Make a 2-column-wide figure if room. See my suggestion to remove (b).}
  % \mike{Normalized maximum cycles $\rightarrow$ Normalized execution cycles (we explained in Methodology how we compute them using max)}

  \caption{Comparing \neat with \mesi, \sarc, and \vips for Phoenix programs that have false sharing detected on 32 cores. Execution time, energy and energy--delay product (EDP) are normalized to \mesi.}
  % Execution time breakdown in (b) is normalized to 100\%.}
  \label{fig:perf-energy-fs}
\end{figure*}

==> figure-performance.tex <==
\begin{figure*}[t!]
  \centering
  \vspace*{-2.5em}
  %\hspace*{12em}\includegraphics[width=0.8\linewidth]{figs/legend_perf}
  %\vspace*{-2.5em}\\
  \subfloat[Execution time]
  {\hspace*{-1.2em}\includegraphics[width=0.8\linewidth]{figs/isca20/max_BandwidthDrivenCycleCountMax}\label{fig:perf}}
	\vspace*{-1.5em}

  \hspace*{6em}\includegraphics[width=0.8\linewidth]{figs/legend_energy}
  \vspace*{-2em}\\
  \subfloat[Energy usage of the cache and memory subsystem]
  {\hspace*{-1.2em}\includegraphics[width=0.8\linewidth]{figs/isca20/TotalEnergy} \label{fig:energy}}
  \vspace*{-1.5em}
  
  \subfloat[Energy--delay product (EDP)]
  {\hspace*{-1.2em}\includegraphics[width=0.8\linewidth]{figs/isca20/EDP} \label{fig:edsp}}
\rui{TODO's: move texts out of bars. \\ change configuration names (discarding any use of the term "opt").}
%     \rui{Will adjust the legend later after we decide on the config/component names.}
% 
%     \mike{As we discussed at some point, I think the traffic graph should be \textbf{non-normalized},
%     using units like GB/s.}
%     \mike{I think that this figure should have three graphs: time, energy, and EDSP.
%     (Non-normalized) traffic should be in a separate figure.}
    %\rui{Changed the config names to be different from the project names.}
%     \rui{Restarted exps for canneal, httpd, memcached and mysqld due to a bug with the phase counters in the \neat/\sarc simulator, which led to wrongly low cycle bars in (a).
%     \\
%     Updated the graphs with the lastest results of memcached and mysqld. Canneal and httpd are still running, so I fixed their cycle bars in the way I mentioned in an earilier email sent to Mike.
%     \\
%     So basically, I think we can settle for the current results if new exps cannot finish by the deadline.}
%     \rui{Updated the perf graph with latest results. Energy updates are pending due to unresolved Sniper issues.}
%     \mike{In (a)'s legend, list Normal execution first, to match bar ordering. Swap Commit and Self-invalidation for same reason.
%     \rui{Revised. What about (b)'s legend? It doesn't make sense to swap the yellow and blue bars to match bar ordering without changing the blue bar's label.
%     So any idea of a better one than ``Other dynamic energy''?}}
    % In (b), solid gray for Static energy doesn't match bar's color.}
    
    \caption{Comparing \neat with \mesi, \sarc, and \vips for PARSEC benchmarks on 32 cores. Execution time, energy, and energy--delay product (EDP) are normalized to \mesi.}
  % {\sf \Arc-32 and \pfopt-32 are the same as in Figure~\ref{fig:perf-traffic}.}
  \label{fig:perf-energy}
\end{figure*}

% \begin{figure*}[t]
%   \centering
%   \vspace*{-2.5em}
%  \includegraphics[width=0.8\linewidth]{figs/g_OnChipBWUsage}
% 	\caption{On-chip bandwidth usage for \mesi, \sarc, and \neat for 32 cores.}  
%   \label{fig:bw-usage}
% \end{figure*}

==> figure-servers.tex <==
\begin{figure*}[t!]
  \centering
  \vspace*{-2.5em}
  \hspace*{-1em}
  \subfloat[Execution time]
  {\includegraphics[width=0.62\linewidth]{figs/isca20/servers/max_BandwidthDrivenCycleCountMax}\label{fig:perf-servers}}

  % \vspace*{-1.0em}
	% \hspace*{6em}\includegraphics[width=1.13\linewidth]{figs/legend_perf}
  % \vspace*{-3.0em}\\
  % \hspace*{-1em}
  % \subfloat[Execution time breakdown across all cores]
  % {\includegraphics[width=0.62\linewidth]{figs/isca20/servers/g_BandwidthDrivenCycleCount}\label{fig:perf-breakdown-servers}}

	\vspace*{-1.0em}
	\hspace*{-0.4em}
  \hspace*{7em}\includegraphics[width=0.8\linewidth]{figs/legend_energy}
  \vspace*{-1.5em}\\
  \hspace*{-1em}
  \subfloat[Energy usage of the cache and memory subsystem]
  {\includegraphics[width=0.62\linewidth]{figs/isca20/servers/TotalEnergy} \label{fig:energy-servers}}

  \vspace*{-1.0em}
  \hspace*{-1em}  
  \subfloat[Energy--delay product (EDP)]
  {\includegraphics[width=0.62\linewidth]{figs/isca20/servers/EDP} \label{fig:edsp-servers}}    

% \mike{Fonts in graph are too small. Make a 2-column-wide figure if room. See my suggestion to remove (b).}
% \mike{Normalized maximum cycles $\rightarrow$ Normalized execution cycles (we explained in Methodology how we compute them using max)}

    \caption{Comparing \neat with \mesi, \sarc, and \vips for server programs on 32 cores. Execution time, energy and energy--delay product (EDP) are normalized to \mesi.}
    % Execution time breakdown in (b) is normalized to 100\%.}
  \label{fig:perf-energy-servers}
\end{figure*}

\later{
\begin{figure*}[t]
  \centering
  \vspace*{-2.5em}
   % \includegraphics[width=0.62\linewidth]{figs/g_OnChipBWUsage}
   
%    \mike{Would traffic be a better term than bandwidth usage? I think bandwidth refers to max supported traffic rate?
%    \rui{I prefer bandwidth usage since we ARE showing the actual usage of the max supported/available traffic rate.}}
   \subfloat[PARSEC benchmarks]
  {\includegraphics[width=0.62\linewidth]{figs/isca20/g_OnChipBWUsage}}
  \vspace*{-0.5em}
  \hspace*{-1em}  
  \subfloat[Server programs]
  {\includegraphics[width=0.83\linewidth]{figs/isca20/servers/g_OnChipBWUsage}}
  \rui{The absolute values of the bars are incorrect since I mistakenly used total cycles instead of max cycles for the computation, but the shapes are not affected by the mistake. We decided to remove the bandwidth graphs anyway.}
  \rui{The bandwidth results don't look quite interesting and not sure if we want to include them in the paper. So I doesn't bother to format them at least for now.}
	\caption{Average on-chip bandwidth consumption for \mesi, \sarc, \vips, and \neat for 32 cores.}  
  \label{fig:bw-usage}
\end{figure*}
}

==> ideas.tex <==
\section{Various Ideas and Thoughts}

Based on what we've learned from developing ARC, can we invent cheap support for DRF0?
DeNovoND~\cite{denovond} and MESI are the main competitors here; also the SARC-like work~\cite{sarc-coherence,vips-directoryless-noc-coherence,denovosync}
and release consistency~\cite{release-consistency,treadmarks}.
Would our design be superior to DeNovoND (which is already cheaper than MESI)?

An ARC-like design targeting DRF0 wouldn't need region boundary operations
except for pre-commit and self-invalidation. It could use some optimizations:\brandon{This is true, but the most basic idea of pre-commit and self-invalidation is bound to be quite inefficient.  Our key problem is to describe how the ARC optimizations are the {\em right} ones to make an efficient self-invalidation system}
\begin{itemize}
\item Self-invalidation optimization for dirty lines, \ie, L1/L2 can avoid invalidation of a dirty line if the version indicates no other core wrote to the line.
\item \emph{Cond-invalid} state (requires versions)
\item Per-core write signature: avoid invalidating any line that isn't indicated by the signature
\item Defer write-backs of dirty lines (the LLC knows that the core is the owner).
\end{itemize}
Some of those require maintaining per-line versions, but that seems like a good idea (since it enables those optimizations).
\brandon{We may want to propose a few different designs: maybe one that is more area efficient and more power efficient, but a little slower, and another that is less power and area efficient because it uses more metadata, but avoids more self-inval, so is faster? We need to fight the complexity-haters this time around.}
% %
When a line is evicted from the L1/L2 to LLC, its written-to bytes (but not its
other bytes) need to be written back to the LLC.

\brandon{What is the area/power cost of adding versions?  What is the performance benefit/reduction in self-inval of adding version?  QUantitative reasoning would help here.}
What happens to a version when it's evicted from the LLC? We're back to the same problem we had with ARC.
One possibility is to maintain the ``max version (of any line) evicted from the LLC'' $\mathit{globalEvictedMax}$,
\ie, $\mathit{globalEvictedMax} \gets \max(\mathit{version},\mathit{globalEvictedMax})$ for each LLC-evicted line,
and when a line is brought back into the LLC, assign $\mathit{version} \gets 1 + \mathit{globalEvictedMax}$.
Versions will overflow more quickly in that case.
We can either have long ($>$32-bit) versions or describe efficient version resetting
(I think a global operation that sets all LLC versions to 1 and all L1/L2 versions to 0, might do it).

